Skipper: Improving the Reach and Fidelity of Quantum Annealers by Skipping Long Chains

Quantum Annealers (QAs) operate as single-instruction machines, lacking a SWAP operation to overcome limited qubit connectivity. Consequently, multiple physical qubits are chained to form a program qubit with higher connectivity, resulting in a drastically diminished effective QA capacity by up to 33x. We observe that in QAs: (a) chain lengths exhibit a power-law distribution, a few dominant chains holding substantially more qubits than others; and (b) about 25% of physical qubits remain unused, getting isolated between these chains. We propose Skipper, a software technique that enhances the capacity and fidelity of QAs by skipping dominant chains and substituting their program qubit with two readout results. Using a 5761-qubit QA, we demonstrate that Skipper can tackle up to 59% (Avg. 28%) larger problems when eleven chains are skipped. Additionally, Skipper can improve QA fidelity by up to 44% (Avg. 33%) when cutting five chains (32 runs). Users can specify up to eleven chain cuts in Skipper, necessitating about 2,000 distinct quantum executable runs. To mitigate this, we introduce Skipper-G, a greedy scheme that skips sub-problems less likely to hold the global optimum, executing a maximum of 23 quantum executables with eleven chain trims. Skipper-G can boost QA fidelity by up to 41% (Avg. 29%) when cutting five chains (11 runs).

==> sections/Acknowledgements.tex <==
\section*{Acknowledgements}
This document is an updated version of HPCA 2022 and 2023, which, in
turn, has been derived from two previous conferences, in particular
HPCA 2021 and MICRO 2021, which, in turn, are derived from past MICRO,
HPCA, ISCA, and ASPLOS conferences.


